BIPED: Pedagogically Informed Tutoring System for ESL Education

Large Language Models (LLMs) have a great potential to serve as readily available and cost-efficient Conversational Intelligent Tutoring Systems (CITS) for teaching L2 learners of English. Existing CITS, however, are designed to teach only simple concepts or lack the pedagogical depth necessary to address diverse learning strategies. To develop a more pedagogically informed CITS capable of teaching complex concepts, we construct a BIlingual PEDagogically-informed Tutoring Dataset (BIPED) of one-on-one, human-to-human English tutoring interactions. Through post-hoc analysis of the tutoring interactions, we come up with a lexicon of dialogue acts (34 tutor acts and 9 student acts), which we use to further annotate the collected dataset. Based on a two-step framework of first predicting the appropriate tutor act then generating the corresponding response, we implemented two CITS models using GPT-4 and SOLAR-KO, respectively. We experimentally demonstrate that the implemented models not only replicate the style of human teachers but also employ diverse and contextually appropriate pedagogical strategies.

==> table/instruction_types.tex <==
% \usepackage{multirow}
\begin{table*}[h]
\resizebox{\textwidth}{!}{
    \begin{tabular}{|l|c|c|c|cc|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}{*}{Instruction type}} & \multirow{2}{*}{Description} & \multirow{2}{*}{Input}                         & \multirow{2}{*}{Output} & \multicolumn{2}{c|}{\# Samples}           \\ \cline{5-6} 
    \multicolumn{1}{|c|}{}                                  &                              &                                                &                           & \multicolumn{1}{c|}{Orignial} & Augmented \\ \hline
    1. Tutor act prediction                                 & Predict a tutor act          & Content, Dialogue                                        & Tutor act                 & \multicolumn{1}{c|}{8,304}    & -         \\ \hline
    2. Next response generation                             &                              & Content, Dialogue, Tutor act                             & Tutor response            & \multicolumn{1}{c|}{8,304}    & 401       \\ \hline
    3. Previous response generation                         &                              & Content, Dialogue \textbackslash Last repsonse, Response & Speaker, Last response    & \multicolumn{1}{c|}{8,304}    & -         \\ \hline
    4. Content based reponse generation                     &                              & Content, Tutor act                             & Tutor response            & \multicolumn{1}{c|}{-}        & 203       \\ \hline
    \end{tabular}
\normalsize}
\caption{A simple description of instruction types for fine-tuning model.}
\label{table:instruction_type}
\end{table*}

% \begin{table*}[h]
% \small
% \centering
% \begin{tabularx}{\textwidth}{XXXXX}
% % {l|c|c|c|cc}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Instruction type}} & \multirow{2}{*}{Description} & \multirow{2}{*}{Input}                         & \multirow{2}{*}{Response} & \multicolumn{2}{c|}{\# Samples}           \\ \cline{5-6} 
% \multicolumn{1}{|c|}{}                                  &                              &                                                &                           & \multicolumn{1}{c|}{Orignial} & Augmented \\ \hline
% 1. Tutor act prediction                                 & Predict a tutor act          & Context                                        & Tutor act                 & \multicolumn{1}{c|}{8,304}    & -         \\ \hline
% 2. Next response generation                             &                              & Context, Tutor act                             & Tutor response            & \multicolumn{1}{c|}{8,304}    & 401       \\ \hline
% 3. Previous response generation                         &                              & Context \textbackslash Last repsonse, Response & Speaker, Last response    & \multicolumn{1}{c|}{8,304}    & -         \\ \hline
% 4. Content based reponse generation                     &                              & Content, Tutor act                             & Tutor response            & \multicolumn{1}{c|}{-}        & 203       \\ \hline
% \end{tabularx}
% \end{table*}

% \begin{table*}[h]
% \small
% \centering
% \begin{tabularx}{\textwidth}{XXXXX}
% \hline
% \textbf{Metric} & \textbf{TSCC v2 \cite{caines2022teacher}} & \textbf{TalkMoves \cite{suresh2022talkmoves}} & \textbf{NCTE \cite{demszky2022ncte}} & \textbf{Ours} \\ \hline
% \# tutoring sessions & 260 & 567 & 1,660 & 112 \\
% \# tutors & 2 & - & 317 & 4 \\
% \# students & 13 & - & 10,817 & 60 \\
% Avg. turns per session & 159.5 & 211.2 & 350 & 105.7 \\
% Avg. words per turn	& T 10.8 / S 6.4 & T 8.2 / S 5.9	& T 29.1 / S 4.0 & T 31.7 / S 8.2 \\
% \# dialogue acts & T,S 12 & T 6 / S 4 & T 3 / S 2 & T 34 / S 9 \\
% domain & ESL & math & math & ESL \\
% setting & 1:1 & classroom & classroom & 1:1 \\ \hline
% \end{tabularx}
% \end{table*}
